Learning to Segment Actions from Observation and Narration

We apply a generative segmental model of task structure, guided by narration, to action segmentation in video. We focus on unsupervised and weakly-supervised settings where no action labels are known during training. Despite its simplicity, our model performs competitively with previous work on a dataset of naturalistic instructional videos. Our model allows us to vary the sources of supervision used in training, and we find that both task structure and narrative language provide large benefits in segmentation quality.

==> datasets.tex <==
\section{Datasets}

\paragraph{CrossTask}
\cite{zhukov2019cross}
Videos from YouTube. 18 primary tasks (annotated), 65 related tasks (unannotated). 2.7K videos in primary; 1.9K additional in related. Has narration, aligned to the video (but noisy).
\df{while this dataset is larger than Breakfast, it's much more diverse}
\an{Note that larger datasets are available (are they?) now.}









==> old-results.tex <==
\section{Results}

\subsection{Supervised framewise}
We compare the frame classifiers, trained in a supervised setting in \autoref{tbl:framewise}. The Gaussian mixture generative models in the top block, which all use PCA-reduced I3D and ResNet features, approach the performance of the discriminative models (including the multi-layer perceptron, MLP, model) which use the full I3D and ResNet features (second block). The Flow model, which learns a Gaussian mixture on top of PCA features produced by a NICE generative flow (jointly learning the parameters of the mixture and the flow), does not improve on the Gaussian mixtures without the flow.

\begin{table*}
    \centering
  \begin{tabular}{lcccc}
    \toprule
    & All-Frame & Step-Frame & Step & Single-Frame \\
    Model & F1 & F1 & Recall & SR \\
    \midrule
    Generative-Full-Sep & 73.1&30&25.1&16.6 \\
Generative-Full-Tied & 74.2&42.4&59&36 \\
Generative-Diag-Sep & 64.3&35.8&65&29.4 \\
Generative-Diag-Tied & 71.9&40.4&60&35.4 \\
\midrule
Disc.Clustering-Shared-Affine & 77.1 & 40.4 & 44 & 31.6 \\
Disc.Clustering-Shared-MLP & 77.6 & 42.8 & 45.0 & 32.9 \\
\midrule
Flow+Generative & 74.2 & 36.1 & 47.7 & 29.7 \\
    \bottomrule
  \end{tabular}
  \caption{\label{tbl:framewise}Framewise classification results for the various featurization models $\phi$. \red{todo: results for the Video-MLP model, showing it's not any better than Shared-MLP}}
\end{table*}

\subsection{Structured Model}

\begin{table*}
    \centering
  \begin{tabular}{llcccc}
    \toprule
    & & All-Frame & Step-Frame & Step & Single-Frame \\
    & & F1 & F1 & Recall & SR \\
    \midrule
    \multicolumn{2}{l}{\cite{zhukov2019cross} published - Sup} &  -- & -- & 31.6 & 31.6 \\
    \multicolumn{2}{l}{\cite{zhukov2019cross} modified - Sup} & 76.2 & 35.1 & 51.4 & 48.0 \\
    \midrule
    Feature function, $\phi$ & Covariance & \\
    \midrule
    PCA & Full-Sep & 73.1 & 27.0 & 27.3 & 18.3 \\
    PCA & Full-Tied &  64.6 & 39.6 & 57.5 & 30.0 \\
    PCA & Diag-Tied & 62.0 & 38.6 & 59.2 & 28.9 \\
\midrule
Disc.Clustering-Shared-Affine & Diag-Tied & 65.7 & 41.6 & 58.0 & 30.3   \\
Disc.Clustering-Shared-MLP & Diag-Tied & 73.9 & 42.4 & 48.9 & 32.7  \\
\midrule
Flow & Diag-Tied & 60.1 & 36.9 & 58.5 & 24.8  \\
    \bottomrule
  \end{tabular}
  \caption{\label{tbl:structured_supervised}Supervised structured classification results using various featurization models $\phi$, and in comparison to past work.}
\end{table*}

See \autoref{tbl:structured_supervised} for a comparison of various feature functions and covariance settings under supervised training of the structured semi-Markov model. Performance varies substantially depending on how the Gaussian mixture covariances are parameterized. \red{this needs to be explored more} Unsurprisingly, using a discriminative clustering model for the features (Disc.Clustering-Shared-Affine) improves performance. As in the framewise setting, we didn't observe an improvement from the Flow featurization, and didn't experiment with it further.

See \autoref{tbl:supervision} for a comparison of various feature functions and supervised and unsupervised training methods in a setting where all frames need to be predicted. All discriminative clustering feature function results use supervised clusters, as joint unsupervised training of the clustering function and structure failed to work in our initial experiments when the background needs to be predicted (see below for these results in a simpler setting without background). When using both the PCA features and supervised clustering features, EM substantially decreases the performance of a supervised model (Supervised vs EM-Supervised Init.), but performance is (as expected) better for the supervised features. More interestingly, supervising the features also leads to a better correlation between likelihood of the model and the F1 metric (results not shown): when using supervised features, EM-Supervised Init. often obtains higher likelihood than EM-Heuristic Init., while with PCA features, EM-Heuristic nearly always has higher log likelihood (but lower F1) than EM-Supervised. This indicates with more discriminative features, we may be able to obtain better task performance through better likelihood optimization (e.g.\ random restarts).

See \autoref{tbl:supervision_oracle_background} for the same experiments but when background is known and only steps need to be predicted (including results for joint learning of the featurization and the structure, \emph{Disc.Clustering-MLP-Joint Unsup}). %

\begin{table*}
    \centering
  \begin{tabular}{lcccc}
    \toprule
    & All-Frame & Step-Frame & Single-Step & Sequence\\
    & Accuracy & Accuracy & Recall & Levenshtein \\
    \midrule
    \multicolumn{5}{l}{\bf Unconstrained / Oracle Assign \df{make sense to put Zhukov here w/ oracle numbers?}} \\
        Uniform baseline -- 72\% background & 56.4 & 11.0 & 16.2 & 47.6 \\
    Richard & \\
    Zhukov & \\
    HMM & \\
    HSMM  & 31.2 & 28.8 & 8.4 & 69.0 \\ %
    \midrule
    \multicolumn{5}{l}{\bf Constraints: Step Ordering} \\
    Uniform baseline -- 0\% background & 6.8 & 24.5 & 8.5 & 73.2 \\
    Uniform baseline -- 72\% background & 55.6 & 8.0 & 11.3 & 45.0 \\
    Richard -- No Narration Cons & \\
    \cite{zhukov2019cross} -- No Narration Cons & 70.2 & 0.6 & 8.0 & 46.1 \\
Cons-HSMM -- No Narration Cons & 52.9 & 9.7 & 9.8 & 45.0  \\
    \midrule
    \multicolumn{5}{l}{\bf Constraints: Step Ordering + Narration In Training} \\
    \cite{zhukov2019cross}  & 70.7 & 1.6 & 22.1 & 45.1 \\
Cons-HSMM & \red{$\approx$ 61} & \red{$\approx$ 16} & \red{$\approx$ 20} & 45.0  \\
    \midrule
    \multicolumn{5}{l}{\bf Constraints: Step Ordering + Narration In Training and Test} \\
    \cite{zhukov2019cross} \\
    Cons-HSMM \\
    \bottomrule
  \end{tabular}
  \caption{\label{tbl:predict_background}Results in the predict-background setting. ``Oracle assign'' indicates prediction labels are assigned to maximize All-Frame accuracy. All results are on the validation set of the CrossTask data. \red{Hidden SMM single-step recall numbers may go up when I implement non-maximal suppression.}}
\end{table*}

\begin{comment}
\begin{table*}
    \centering
  \begin{tabular}{lccc}
    \toprule
    & Step-Frame & Single-Step & Sequence\\
    & Accuracy & Recall & Levenshtein \\
\midrule
    Uniform canonical baseline (oracle assign) & 32.5 & 43.4 & 55.1  \\
Hidden SMM, unconstrained (oracle assign) & 35.6 & 26.5 & 67.6 \\ %
    \midrule
    Uniform canonical baseline & 27.8 & 39.8 & 53.8  \\
    \green{\cite{zhukov2019cross}, adapted, no narr. constraints} & 14.2 & 32.6 & 53.8  \\ %
\green{Hidden SMM, constrained ordering} & 25.0 & 37.9 & 53.8 \\  %
\midrule
    \cite{zhukov2019cross}, adapted & 38.9 & 43.7 & 53.8  \\ %
Hidden SMM, constrained ordering + Narration & 35.3 & 46.0 & 53.8 \\
    \bottomrule
  \end{tabular}
  \caption{\label{tbl:oracle_background}Results in the oracle background setting. ``Zhukov Adapted'' means modified for the oracle background setting. "Oracle assign" indicates prediction labels are assigned to maximize Step-Frame accuracy. All results are on the validation set of the CrossTask data. \red{Zhukov and Hidden SMM single-step recall numbers may go up when I implement non-maximal suppression.}}
\end{table*}
\end{comment}

\begin{table*}
    \centering
  \begin{tabular}{lccc}
    \toprule
    & Step-Frame & Single-Step & Sequence\\
    & Accuracy & Recall & Levenshtein \\
    \midrule
    \multicolumn{4}{l}{\bf Unconstrained / Oracle Assign \df{put Zhukov here w/ oracle numbers?}} \\
    Uniform baseline  & 32.5 & 43.4 & 55.1  \\
    Richard & \\
    Zhukov & \\
    HMM & \\
HSMM & 35.6 & 26.5 & 67.6 \\ %
    \midrule
    \multicolumn{4}{l}{\bf Constraints: Step Ordering} \\
    Uniform baseline & 27.8 & 39.8 & 53.8  \\
    Richard -- No Narration Cons & \\
    \cite{zhukov2019cross} -- No Narration Cons & 14.2 & 32.6 & 53.8  \\ %
Cons-HSMM -- No Narration Cons  & 25.0 & 37.9 & 53.8 \\  %
    \midrule
    \multicolumn{4}{l}{\bf Constraints: Step Ordering + Narration In Training} \\
    \cite{zhukov2019cross}, adapted  & 38.9 & 43.7 & 53.8  \\ %
Cons-HSMM &  35.3 & 46.0 & 53.8 \\
    \midrule
    \multicolumn{4}{l}{\bf Constraints: Step Ordering + Narration In Training and Test} \\
    \cite{zhukov2019cross}, adapted \\
    Cons-HSMM \\
    \bottomrule
  \end{tabular}
  \caption{\label{tbl:predict_background}Results in the oracle background setting. ``Zhukov Adapted'' means modified for the oracle background setting. "Oracle assign" indicates prediction labels are assigned to maximize Step-Frame accuracy. All results are on the validation set of the CrossTask data. \red{Zhukov and Hidden SMM single-step recall numbers may go up when I implement non-maximal suppression.}}
\end{table*}


\begin{comment}
\begin{table*}
    \centering
  \begin{tabular}{llcccc}
    \toprule
    & & All-Frame & Step-Frame & Step & Single-Frame \\
    & & F1 & F1 & Recall & SR \\
    \midrule
    \multicolumn{2}{l}{\cite{zhukov2019cross} modified - Unsup} & 70.7 & 35.1 & 51.4 & 48.0 \\
    \multicolumn{2}{l}{\cite{richard2018action} - Unsup} & 42.1 & 13.5 & 34.1 & 15.5 \\
    \midrule
    Feature function, $\phi$ & Training & \\
    \midrule
    PCA & Supervised & 62.0 & 38.6 & 59.2 & 28.9 \\
    PCA & EM-Supervised Init. & 38.4 & 22.6 & 41.3 & 12.6 \\
    PCA & EM-Heuristic Init. & 28.0 & 18.0 & 33.6 & 9.5 \\
\midrule
Disc.Clustering-Shared-MLP-Sup & Supervised & 73.9 & 42.4 & 48.9 & 32.7  \\
Disc.Clustering-Shared-MLP-Sup & EM-Supervised Init. & 57.9 & 29.3 & 52.7 & 30.2 \\
Disc.Clustering-Shared-MLP-Sup & EM-Heuristic Init. & 44.6 & 24.5 & 56.6 & 27.4 \\
\midrule
    \bottomrule
  \end{tabular}
  \caption{\label{tbl:supervision}Structured classification results comparing forms of supervision in training, and in comparison to past work. All models use Diag-Tied covariance matrices. The feature representations for the discriminative clustering model (Disc.Clustering-Shared-MLP-Sup) are supervised.}
\end{table*}

\begin{table*}
    \centering
  \begin{tabular}{llccc}
    \toprule
    & & Step-Frame & Step & Single-Frame \\
    & & F1 & Recall & SR \\
    \midrule
    \multicolumn{2}{l}{\cite{richard2018action} - Unsup} & 32.7 & 64.9 & 45.2 \\
    \midrule
    Feature function, $\phi$ & Training & \\
    \midrule
    PCA & Supervised &  62.8 & 66.4 & 50.0 \\
    PCA & EM-Supervised Init. & 47.0 & 46.7 & 30.3 \\
    PCA & EM-Heuristic Init. & 37.5 & 38.4 & 22.3 \\
\midrule
Disc.Clustering-Shared-MLP-Sup & Supervised & 68.9 & 68.7 & 52.4 \\
Disc.Clustering-Shared-MLP-Sup & EM-Supervised Init. & 68.1 & 69.9 & 53.8 \\
Disc.Clustering-Shared-MLP-Sup & EM-Heuristic Init. & 53.7 & 64.9 & 47.6 \\
Disc.Clustering-Shared-MLP-Joint Unsup & EM-Heuristic Init. & 40.0 & 41.2 & 23.7 \\
\midrule
    \bottomrule
  \end{tabular}
  \caption{\label{tbl:supervision_oracle_background}Oracle background structured classification results comparing forms of supervision in training, and in comparison to past work. For the discriminative clustering model, \emph{-Sup} indicates the feature representations are supervised; \emph{-Joint Unsup} are unsupervised and jointly learned with the structure (Sec.~\ref{sec:joint_training}).}
\end{table*}

\end{comment}
